COVID-19 Outbreak Prediction and Analysis using Self Reported Symptoms

It is crucial for policymakers to understand the community prevalence of COVID-19 so combative resources can be effectively allocated and prioritized during the COVID-19 pandemic. Traditionally, community prevalence has been assessed through diagnostic and antibody testing data. However, despite the increasing availability of COVID-19 testing, the required level has not been met in most parts of the globe, introducing a need for an alternative method for communities to determine disease prevalence. This is further complicated by the observation that COVID-19 prevalence and spread varies across different spatial, temporal, and demographics. In this study, we understand trends in the spread of COVID-19 by utilizing the results of self-reported COVID-19 symptoms surveys as an alternative to COVID-19 testing reports. This allows us to assess community disease prevalence, even in areas with low COVID-19 testing ability. Using individually reported symptom data from various populations, our method predicts the likely percentage of the population that tested positive for COVID-19. We do so with a Mean Absolute Error (MAE) of 1.14 and Mean Relative Error (MRE) of 60.40\% with 95\% confidence interval as (60.12, 60.67). This implies that our model predicts +/- 1140 cases than the original in a population of 1 million. In addition, we forecast the location-wise percentage of the population testing positive for the next 30 days using self-reported symptoms data from previous days. The MAE for this method is as low as 0.15 (MRE of 23.61\% with 95\% confidence interval as (23.6, 13.7)) for New York. We present an analysis of these results, exposing various clinical attributes of interest across different demographics. Lastly, we qualitatively analyze how various policy enactments (testing, curfew) affect the prevalence of COVID-19 in a community.

==> ablation_studies.tex <==
\section{Ablation Studies}

Here, we perform ablation studies to verify and investigate the relative importance of the features that were selected using f regression feature ranking algorithm\cite{Freg}. In the following experiments the top $N=10$ features obtained from the f regression algorithm are considered as the subset for evaluation.
\\

\textbf{All-but-One}:
In this experiment, the target variable which is the percentage of people affected by COVID 19 is estimated by considering $N-1$ features from a given set of top $N$ features by dropping 1 feature at a time in every iteration in a descending order. The results are visualised in figure \ref{fig:mre_vs_ifr} from which it is clear that there is a considerable increase error when the most significant feature is dropped and the loss in performance is not as drastic when any other feature is dropped. This reaffirms that our feature selection method is valid.
\\
\begin{comment}


\begin{figure}
    \includegraphics[width=\linewidth]{pca_plots/MAEvIFR.png}
    \caption{results of All-but-One experiment (MAE)}
    \label{fig:mae_vs_ifr}
\end{figure}
\end{comment}
\begin{figure}[t!]
    \includegraphics[width=\linewidth]{pca_plots/MREvIFR.png}
    \caption{Results of All-but-One experiment (MRE)}
    \label{fig:mre_vs_ifr}
\end{figure}




\textbf{Cumulative Feature Dropping}: 
In this experiment, we estimate the target variable based on top $N$=10 features and then carry out the experiment with $N-i$ features in every iteration where $i$ is the iteration count. The features are dropped in the descending order. Figure \ref{fig:re_fr} shows the results. The change in slope from the start to the end of the graph strongly supports our previous inference that the most important feature has a huge significance on the performance and error rate and reaffirms our features selection algorithm.\newline
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{pca_plots/RE_FR.png}
    \caption{Results of Cumulative Feature Dropping}
    \label{fig:re_fr}
\end{figure}


==> done.tex <==

     
\section{Completed Tasks}
\begin{itemize}
    \item Processing UMD Dataset - Rohan
    \item Processing CMU Dataset - Sheshank
    \item Trying basic models on CMU Dataset - Sheshank: This is giving a suspiciously high accuracy rate so we need to work on removing some highly correlated features
    \item Modeling the UMD dataset as time-series - Rohan
    \item DL model for timeseries forecast - Rohan
    
    \item select k best features using univaritate techiques -parth
    \item regression algos - parth
    \item PCA - Sheshank
    
    
\end{itemize}

==> related_work.tex <==
\section{Related Work}

Due to the massive amount of COVID-19 data available and the need to make sense of this data quickly, a variety of Machine Learning algorithms have been applied to help researchers gain essential answers such as forecasting the number of cases, identifying symptoms associated to the disease and understanding how policies affect the spread of the virus.\\
Methods focused on identifying the symptoms such as Parma et al.[3] study the impact of COVID-19 on the sensory-nasal symptoms showing that COVID-19 impairs the sense of smell, taste and chemesthesis. Menni et al. used self reported data from a mobile app to predict COVID-19 positivity using symptoms. They found anosmia to be the strongest predictor of disease presence, and were able to generate a symptoms based model for disease detection with a sensitivity of ~.65. \\ 
Ribeiro et al.[4] evaluated various forecasting models such as ARIMA, CUBIST, RIDGE etc. to forecast the number of cases in the context of Brazil. Chinmula et al.[5] have worked on a similar study in the context of Canada where they utilize LSTM networks to predict trends as well as the possible stopping times.
Governments and various other policy making bodies around the world have also introduced various measures and policies to combat the spread of virus. Hsiang et al. have studied the impact of policies introduced by the policy makers in China, South Korea, Italy, Iran, France and the United States on the infection rates. Lyu et al. report their findings on how introducing state mandated masks helped reduce the number of cases by more than 200,000 cases by May 2020.



==> sections.tex <==
abstract - Sheshank done
intro sheshank, joseph done

related works yash done

dataset - sheshank

Method:
    umd time series Rohan done
    cmu time series Rishank
    cmu prediction Parth done
    cmu correlation Sethu
   
 
Result and discussion
    umd time series Rohan
    cmu prediction Parth
    cmu correlation Sethu
    cmu time series Rishank 
    
    
Conclusion and future abhishek


pending
mortality, wildfire??

==> signal_ablation.tex <==
\section{Signal Ablation}
I'm not sure how much of this we'll actually use, but I thought it would be good to add it all in here for now.

These are some experiments showing some relationships that we already know

\subsection{Shortness of Breath and Sore throat v.s. Positive COVID Case}
\includegraphics[width=3in]{pca_plots/pca.png}

Running a 2 layer fully connected neural network is able to predict positive COVID case with an error of 0.08%.

\subsection{Pre-existing Medical Conditions v.s. Positive COVID Case}
\includegraphics[width=3in]{pca_plots/pre-existing_medical_conditions.png}

This graph shows that pre-existing medical conditions do not appear to make people more susceptible to the virus.

check mortality vs pre-existing conditions.

